Biological Random Walks: integrating heterogeneous data in disease gene prioritization

This work proposes a unified framework to leverage biological information in network propagation-based gene prioritization algorithms. Preliminary results on breast cancer data show significant improvements over state-of-the-art baselines, such as the prioritization of genes that are not identified as potential candidates by interactome-based algorithms, but that appear to be involved in/or potentially related to breast cancer, according to a functional analysis based on recent literature.

==> trunk/todo <==
- Ricordarsi di citare Mirtabase tra le sorgenti biologiche nella Sez. II
- Ricordarsi di accennare a grid-search
    
- Aggiungere tabella /statistiche brw vs all, per far capire che abbiamo girato un sacco di esperimenti
- rimuovere parte diamond
- aggiungere spiegazione enriched set
- forse reimposterei materials e method cosi:
    - diamo subito la scelta ottimale della pipeline di  BRW, quindi l'inverse sigmoid ranking, t=1 etc...
    - e poi spiegherei che in verità abbiamo provato molteplici combinazioni di funzioni


BRW: biological random walk for disease gene prioritization






AUTHORS


\IEEEauthorblockN{ Michele Gentili}
\IEEEauthorblockA{\textit{DIAG department \footnote{Department of Computer,Control, and Management Engineering Antonio Ruberti}} \\
\textit{University of Rome}\\
Rome, Italy \\
gentili@diag.uniroma1.it}
\and
\IEEEauthorblockN{ Leonardo Martini}
\IEEEauthorblockA{\textit{Department of Computer,} \\ \textit{Control, and Management Engineering} \\ \textit{Antonio Ruberti} \\
\textit{University of Rome}\\
Rome, Italy \\
martini@diag.uniroma1.it}
\and
\IEEEauthorblockN{Manuela Petti}
\IEEEauthorblockA{\textit{Department of Computer,} \\ \textit{Control, and Management Engineering} \\ \textit{Antonio Ruberti} \\
\textit{University of Rome}\\
Rome, Italy \\
petti@diag.uniroma1.it}
\and
\IEEEauthorblockN{Lorenzo Farina}
\IEEEauthorblockA{\textit{Department of Computer,} \\ \textit{Control, and Management Engineering} \\ \textit{Antonio Ruberti} \\
\textit{University of Rome}\\
Rome, Italy \\
farina@diag.uniroma1.it}
\and
\IEEEauthorblockN{Luca Becchetti}
\IEEEauthorblockA{\textit{Department of Computer,} \\ \textit{Control, and Management Engineering} \\ \textit{Antonio Ruberti} \\
\textit{University of Rome}\\
Rome, Italy \\
becchetti@diag.uniroma1.it}
\and
